Low-Power Wide-Area Network Design

LPWAN is an enabling technology for long-range, low-power, and low-cost IoT/CPS applications. Recently, multiple LPWAN technologies have been developed that operate in the licensed (e.g., 5G) and ISM (e.g., LoRa) bands. To avoid the crowd in the ISM band and the cost of the licensed band, we propose a novel LPWAN called Sensor Network Over White Spaces (SNOW) by utilizing the TV white spaces. Specifically, we design, develop, and experiment SNOW, which is highly scalable, energy-efficient, and has a long communication range. SNOW achieves scalability and energy efficiency by enabling concurrent packets reception at a BS using a single radio from numerous sensors and concurrent packets transmission to numerous sensors from the BS using a single radio, simultaneously, which we achieve by proposing a distributed implementation of OFDM. To enable the low-cost and scalable SNOW deployment in practical applications, we implement SNOW using the low-cost and small form-factored COTS devices, where we address multiple practical challenges including the high peak-to-average power ratio, channel state estimation, and carrier offset estimation. Also, we propose an adaptive transmission power protocol to handle the near-far power problem. To enable connecting tens of thousands of nodes over hundreds of kilometers, we further propose a network architecture called SNOW-tree through a seamless integration of multiple SNOWs where they form a tree structure and are under the same management/control. We address the intra- and inter-SNOW interferences by formulating a constrained optimization problem called the scalability optimization problem (SOP) whose objective is to maximize scalability by managing the spectrum sharing across the SNOWs. By proving the NP-hardness of SOP, we then propose two polynomial-time methods to solve it: a greedy heuristic algorithm and a 1/2-approximation algorithm.

==> autobiographicalStatement.tex <==
%Create bio section with unnumbered section
\section*{AUTOBIOGRAPHICAL STATEMENT}
%
%Add reference to the table of contents {toc} at the section level {section} titled "Autobiographical Statement" {Autobiographical Statement}
\addcontentsline{toc}{section}{Autobiographical Statement}
Md Mahbubur Rahman received a bachelor's degree in Computer Science and Engineering from Bangladesh University of Engineering and Technology, Dhaka, Bangladesh, in 2012. 
He is currently pursuing a Ph.D. degree with the Department of Computer Science, Wayne State University. 
His research interests include Low-Power Wide-Area Networks, Internet of Things, Cyber-Physical Systems, Wireless Sensor Networks, and Distributed Systems. He has co-primary-authored a paper that was nominated for the best paper award at ACM SenSys 2016. In 2019, he received the Michael E. Conrad Outstanding Graduate Research Publication Award for publishing the most significant research article in the field of Computer Science at Wayne State University. He has also published many research articles in the top-tier conferences and journals of Computer Science.


